OceanGym: A Benchmark Environment for Underwater Embodied Agents

We introduce OceanGym, the first comprehensive benchmark for ocean underwater embodied agents, designed to advance AI in one of the most demanding real-world environments. Unlike terrestrial or aerial domains, underwater settings present extreme perceptual and decision-making challenges, including low visibility, dynamic ocean currents, making effective agent deployment exceptionally difficult. OceanGym encompasses eight realistic task domains and a unified agent framework driven by Multi-modal Large Language Models (MLLMs), which integrates perception, memory, and sequential decision-making. Agents are required to comprehend optical and sonar data, autonomously explore complex environments, and accomplish long-horizon objectives under these harsh conditions. Extensive experiments reveal substantial gaps between state-of-the-art MLLM-driven agents and human experts, highlighting the persistent difficulty of perception, planning, and adaptability in ocean underwater environments. By providing a high-fidelity, rigorously designed platform, OceanGym establishes a testbed for developing robust embodied AI and transferring these capabilities to real-world autonomous ocean underwater vehicles, marking a decisive step toward intelligent agents capable of operating in one of Earth's last unexplored frontiers. The code and data are available at https://github.com/OceanGPT/OceanGym.

==> table/comparison.tex <==
\begin{table}[h]
    \centering
    \caption{Comparison of other benchmarks}
    \scalebox{0.85}{
    \begin{tabular}{lllcl}
        \toprule
        \textbf{Benchmark} & \textbf{Environment} & \textbf{Motion} & \textbf{Simulator} & \textbf{Sensing}\\
        \midrule
        Room-to-Room \citep{r2r} & Indoor & Ground-Level & \checkmark & RGB\\
        RoomNav \citep{House3D} & Indoor & Ground-Level & \checkmark & RGB\\
        TOUCHDOWN \citep{Touchdown} & Outdoor & Ground-Level & $\times$ & RGB\\
        NuScenes \citep{NuScenes} & Street & Ground-Level & $\times$ & RGB/Lidar/Radar\\
        Talk2Nav \citep{Talk2Nav} & Outdoor & Ground-Level & \checkmark & RGB\\
        HourVideo \citep{hourvideo} & Indoor/Outdoor & Ground-Level & $\times$ & RGB\\
        EgoSchema \citep{egoschema} & Indoor/Outdoor & Ground-Level& $\times$ & RGB\\
        Lingoqa \citep{lingoqa} & Street & Ground-Level & $\times$ & RGB\\
        CityNav \citep{CityNav} & City & Aerial Space & \checkmark & RGB/GPS/Pose\\
        OpenUAV \citep{OpenUAV} & City & Aerial Space & \checkmark & RGB\\
        OpenFly \citep{OpenFly} & City & Aerial Space & \checkmark & RGB\\     
        UrbanVideo-Bench \citep{UrbanVideo} & City & Aerial Space & $\times$ & RGB\\
        \midrule
        Ours & Underwater & Underwater Space & \checkmark & RGB/GPS/Sonar\\
        \bottomrule
    \end{tabular}
    }
\label{tab:comparison}
\end{table}

==> table/decision_more_methods.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.95}{
\begin{tabular}{@{}l*{5}{c}c@{}}
\toprule
\multirow{2}{*}{Task} & \multicolumn{5}{c}{Method / Model} & \multirow{2}{*}{Human} \\
\cmidrule(lr){2-6}
& GLM-4.5V & GPT-4o-mini & Gemini-2.5 & Qwen2.5-VL-7B & Outward spiral \\
\midrule
Inspect the oil pipe (Shallow) & $37.8_{\color{gray}\pm 17.88}$ & $27.1_{\color{gray}\pm 23.6}$ & $18.3_{\color{gray}\pm 15.8}$ & $30.8_{\color{gray}\pm 25.2}$ & $33.3_{\color{gray}\pm 29.8}$ & 100 \\
Inspect the oil pipe (Deep) & $32.5_{\color{gray}\pm 5.86}$ & $15.8_{\color{gray}\pm 15.5}$ & $6.6_{\color{gray}\pm 11.4}$ & $21.7_{\color{gray}\pm 25.3}$ & $9.42_{\color{gray}\pm 19.48}$ & 78.2 \\
\bottomrule
\end{tabular}
}
\caption{Performance comparison between traditional algorithms and models for ``Inspect the oil pipe'' task.}
\label{tab:decision_more_methods}
\end{table*}

==> table/decision_prompt.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.95}{
\begin{tabular}{@{}lc@{}}
\toprule
Task & GPT-4o-mini \\
\midrule
\textbf{\makecell{Shallow Water Environment (High Illumination)}} & \\
\midrule
Search for a sunken ship (Prompt 1) & $\underline{13.4}_{\color{gray}\pm 19.3}$ \\
Search for a sunken ship (Prompt 2) & $\underline{12.5}_{\color{gray}\pm 13.6}$ \\
\bottomrule
\end{tabular}
}
\caption{Performance of decision tasks across different prompts.}
\label{tab:decision_prompt}
\end{table*}

==> table/more_tasks.tex <==
\begin{table*}[t]
\centering
\small
\scalebox{0.96}{
\begin{tabular}{@{}lccccc@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{\makecell{Shallow Water Environment\\(High Illumination)}} & \multicolumn{2}{c}{\makecell{Deep Water Environment\\(Low Illumination)}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & Vision & Vision+Sonar & Vision & Vision+Sonar \\
\midrule
GPT-4o-mini (85 scenes) & 29.41 & 34.12 & 10.59 & 15.29 \\
GPT-4o-mini (100 scenes) & 33.00 & 37.00 & 17.00 & 21.00 \\
GPT-5.2 (85 scenes) & 49.41 & 62.35 & 28.24 & 35.29 \\
GPT-5.2 (100 scenes) & 51.00 & 61.00 & 33.00 & 38.00 \\
Gemini-3-Pro (85 scenes) & 52.94 & 60.00 & 38.82 & 37.65 \\
Gemini-3-Pro (100 scenes) & 48.00 & 59.00 & 36.00 & 40.00 \\
\bottomrule
\end{tabular}}
\caption{Comparison of results across more perception tasks.}
\label{tab:more_tasks}
\end{table*}

==> table/prompt.tex <==
\begin{table*}[h]
\centering
\small
\scalebox{0.99}{
\begin{tabular}{@{}l*{10}{c}@{}}
\toprule
\multirow{3}{*}{Model} & \multicolumn{5}{c}{\makecell{Shallow Water Environment\\(High Illumination)}} & \multicolumn{5}{c}{\makecell{Deep Water Environment\\(Low Illumination)}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
 & \multicolumn{2}{c}{\makecell{Multi-View\\Perception}} & \multicolumn{2}{c}{\makecell{Context-based\\Perception}} & \multirow{2}{*}{Avg} & \multicolumn{2}{c}{\makecell{Multi-View\\Perception}} & \multicolumn{2}{c}{\makecell{Context-based\\Perception}} & \multirow{2}{*}{Avg} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
 & Vision & +Sonar & Vision & +Sonar & & Vision & +Sonar & Vision & +Sonar & \\
\midrule

GPT-4o-mini(prompt1) & 34.55 & 34.55 & 20.00 & 33.33 & 30.61 & 14.55 & 20.00 & 3.33 & 6.67 & 11.14 \\
GPT-4o-mini(prompt2) & 54.55 & 45.45 & 40.00 & 30.00 & 42.5 & 20.00 & 20.00 & 10.00 & 0.00 & 12.5 \\
\bottomrule
\end{tabular}}
\caption{Performance of perception tasks across different prompts.}
\label{tab:prompt}
\end{table*}
